Securing Smart Contract On The Fly

We present Solythesis, a source to source Solidity compiler which takes a smart contract code and a user specified invariant as the input and produces an instrumented contract that rejects all transactions that violate the invariant. The design of Solythesis is driven by our observation that the consensus protocol and the storage layer are the primary and the secondary performance bottlenecks of Ethereum, respectively. Solythesis operates with our novel delta update and delta check techniques to minimize the overhead caused by the instrumented storage access statements. Our experimental results validate our hypothesis that the overhead of runtime validation, which is often too expensive for other domains, is in fact negligible for smart contracts. The CPU overhead of Solythesis is only 0.12% on average for our 23 benchmark contracts.

==> __latexindent_temp.tex <==
@misc{dao,
title={Analysis of the DAO exploit},
howpublished={\url{http://hackingdistributed.com/2016/06/18/analysis-of-the-dao-exploit/}},
author={Daian, Phil},
year={2016},
month={Jun}
}

==> figures/__latexindent_temp.tex <==
      &pre\leftarrow(\mathrm{if}\;(e_3')\;

==> figures/aggregate-decoration.tex <==
\Input{assignment statement $s$, list of aggregates $K$}
\Output{instrumented assignment statement $s$, assertions statements $\alpha$}
\underline{function} $\mathrm{visit}(s, K):$\\
\Begin{
$v\leftarrow\mathrm{getStateVar(getLeftHandSide(s))}$

$\alpha\leftarrow \emptyset$

\For {$s'\in K$} {
  \If {$v\not\in s'$} {
    \Continue
  }
  $\mathrm{instrument}$($s',s,\alpha,K$)
}
\Return $s,\alpha$
}

==> figures/constraint-collection.tex <==
\Input{function node $f$, call graph $G$}
\Output{a set of assertion statements $\alpha$}
\underline{function} $\mathrm{collectAssertions}(f, G):$\\
\Begin{
$\alpha\leftarrow\emptyset$

$\zeta\leftarrow f\cdot[\,]$

$\theta\leftarrow \{f\}$


\While {$\zeta\not=[\,]$} {
  $f'\cdot \zeta'\leftarrow \zeta$

  $\alpha\leftarrow\mathrm{getAssertionStatments}(f');\;\alpha$

  \For {$f'' \in \mathrm{predecessor}(f', G)$} {

    \If {$f''\not\in\theta$} {
      $\zeta'\leftarrow\zeta'\cdot f$

      $\theta\leftarrow\theta\cup f$
    }
  }
  $\zeta\leftarrow\zeta'$
}
\Return $\alpha$
}

==> figures/constraint-decoration.tex <==
\Input{constraints $\kappa$}
\Output{list of assertions $s$}
\underline{function} $\mathrm{translateConstraints}(\kappa):$\\
\Begin{
$stmts \leftarrow [\,]$

\For {$c\in\kappa$} {
  \Switch {$c$} {
    \Case {$\mathrm{constraint}\;e$} {
      $stmts\leftarrow stmts\cdot\mathrm{assert}(e)$
    }
    \Case {$\mathrm{constraint\;forall}(\vv{\mu},e)$} {
      $stmts\leftarrow stmts\cdot(index=0)$

      $v\leftarrow \mathrm{stateVarInContract}(\vv{\mu}_0)$

      $stmts\leftarrow stmts\cdot(length=v.length)$

      $\psi\leftarrow \emptyset$

      \For {$\mu\in\vv{\mu}$} {
        $v\leftarrow \mathrm{stateVarInContract}(\mu)$

        $\psi[\mu\leftarrow v_{index}]$
      }

      $e'\leftarrow\mathrm{rewrite}(\psi, e)$

      $s\leftarrow \mathrm{assert}(e');index+=1$

      $stmts\leftarrow stmts\cdot\mathrm{while}\;(index<length)\; s$
    }
  }
  \Return stmts
}
}

==> figures/rewrite-rules.tex <==
\begin{align*}
\begin{split}
    s'&:=v=\mathrm{sum}(\vv{\mu_1}, \vv{\mu_2}, e_1, e_2, e_3)\quad s\quad\alpha\quad K\\[1pt]
    \hline\\[-10pt]
    \psi&\leftarrow\mathrm{bind}(s', s)\\
    e_1'&\leftarrow\mathrm{rewrite}(e_1, \psi)\\
    e_2'&\leftarrow\mathrm{rewrite}(e_2, \psi)\\
    e_3'&\leftarrow\mathrm{rewrite}(e_3, \psi)\\
    pre, \alpha_1&\leftarrow\mathrm{visit}(\mathrm{if}\;(e_3')\;v\llbracket\vv{\mu_1}'\cdot e_2'\rrbracket\minuseq e_1', K)\\
    post, \alpha_2&\leftarrow\mathrm{visit}(\mathrm{if}\;(e_3')\;v\llbracket\vv{\mu_1}'\cdot e_2'\rrbracket\minuseq e_1', K)\\
    \alpha&\leftarrow \alpha;\;\alpha_1;\;\alpha_2\\
    s&\leftarrow pre;\; s;\; post \\\\
    s'&:=\mathrm{constraint\;forall}(\vv{\mu}, e)\quad s\quad \alpha\quad K\\[1pt]
    \hline\\[-10pt]
    \psi&\leftarrow\mathrm{bind}(s', s)\\
    \vv\mu'&\leftarrow\mathrm{rewrite}(\vv\mu, \psi)\\
    \vv v&\leftarrow\mathrm{getStateVarForMu}(\vv\mu)\\
    s&\leftarrow\mathrm{push}(v_0, \mu_0');\;\mathrm{push}(v_1, \mu_1');\;...;\;\\
    &\quad\;\;\mathrm{push}(v_n, \mu_n');\;s\\
    i&\leftarrow\mathrm{createVar}()\\
    \psi'&\leftarrow\left\{
    \begin{array}{ll}
        \mu_0\mapsto v_0\llbracket i\rrbracket\\
        \mu_1\mapsto v_1\llbracket i\rrbracket\\
        ...\\
        \mu_n\mapsto v_n\llbracket i\rrbracket\\
    \end{array}
    \right\}\\
    e'&\leftarrow\mathrm{rewrite}(e, \psi')\\
    s_1&\leftarrow\mathrm{assert}(e');\;i\pluseq 1\\
    s_2&\leftarrow\mathrm{while}(i<\mathrm{length}(v_0))\;s_1\\
    \alpha&\leftarrow\alpha;\;s_2\\\\
    s'&:=\mathrm{constraint\;}e\quad s\quad \alpha\quad K\\[1pt]
    \hline\\[-10pt]
    \alpha&\leftarrow\alpha;\;\mathrm{assert}(e)
    % t\leftarrow& index=v_0.length;\;\mathrm{while}(index < length)\\
    % a\leftarrow& index=v_0.length;\;\mathrm{while}(index < length)\\
\end{split}
\end{align*}


==> figures/state-var.tex <==
\Input{indexing expression $e$}
\Output{state variable}
\underline{function} $\mathrm{getStateVar}(e):$\\
% \Begin{
  \If {\Not $\mathrm{isIndexing}(e)$} {
    \Return $e$
  }
  \Return $\mathrm{getStateVar}(\mathrm{getObjectExpression}(e))$
% }

==> figures/substitution-rule.tex <==
\begin{align*}
\begin{split}
  \mu[t/\mu]&\equiv t\\
  v[t/\mu]&\equiv v\\
  \mu[t/\mu']&\equiv \mu \text{ and }\mu\not\equiv\mu'\\
  (A_1\;aop\;A_2)[t/\mu]&\equiv A_1[t/\mu]\;aop\;A_2[t/\mu]\\
  (A_{1{A_2}})[t/\mu]&\equiv {A_1[t/\mu]}_{{A_2}[t/\mu]}
\end{split}
\end{align*}


==> figures/types.tex <==
\begin{gather*}
    t \in \mathrm{Type} := i\;|\;m \qquad
    i,i_1\in \mathrm{Integer} \\
    m \in \mathrm{Mapping}:=\mathrm{mapping}\;i\;t
\end{gather*}
\begin{align*}
\begin{split}
    &\frac{e_1\oplus e_2}{\Sigma\vdash e_1:\mathrm{Integer}\quad\Sigma\vdash e_2:\mathrm{Integer}} \\\\
    &\frac{\Sigma\vdash e_1:\mathrm{mapping}\;i\;t\quad e_{1e_2}}{\Sigma\vdash e_2:i\quad \Sigma\vdash e_{1e_2}:t}\\\\
    &\frac{\Sigma\vdash \vv{\mu}:\vv{t}\quad v=\mathrm{sum}(\vv{\mu},\bullet,\bullet,\bullet,\bullet)}
    {\Sigma\vdash v:\mathrm{sumtype}\;\vv{t}}
\end{split}
\end{align*}
\begin{align*}
\begin{split}
    \mathrm{sumtype}\;\emptyset&=\mathrm{mapping\;Integer\;Integer} \\
    \mathrm{sumtype}\;t_1\cdot\vv{t}&= \mathrm{mapping}\;t_1\;(\mathrm{sumtype}\;\vv{t})
\end{split}
\end{align*}

==> figures/variablecache.tex <==
\begin{align*}
\begin{split}
    &v=\text{Sum}(\vv{\mu_1}, \vv{\mu_2}, A_1, A_2, B)\quad a \quad M \\
    \hline
    a_{pre}\leftarrow&\\
    &tmp=v_{\vv{\mu_1}[M]A_2[M]} \\
    & if\;(B[M])\quad tmp \mathrel{-}= A_1[M]\\
    & a_{pre}\\
    a_{post}\leftarrow&\\
    & if\;(B[M])\quad tmp \mathrel{+}= A_1[M]\\
    &v_{\vv{\mu_1}[M]A_2[M]}=tmp \\
    & a_{post}
\end{split}
\end{align*}




==> files/__latexindent_temp.tex <==
     \textbf{S}

==> files/appa.tex <==
\section{Error Triggering Input}\label{appendix:error-triggering}

\begin{figure}[t]
\scriptsize
\begin{center}
\begin{tabular}{ |c|c| } 
\hline
Variable & Value \\ 
\hline
\sourcecode{ADDRS.length} & 3 \\ 
\sourcecode{ADDRS[0]} & 0x67518339e369ab3d591d3569ab0a0d83b2ff5198 \\ 
\sourcecode{ADDRS[1]} & 0xd30a286ec6737b8b2a6a7b5fbb5d75b895f62956 \\ 
\sourcecode{ADDRS[2]} & 0x1bfa530d5d685155e98cd7d9dd23f7b6a801cfef \\ 
\sourcecode{sender} & \sourcecode{ADDRS[0]} \\ 
\scriptsize{\sourcecode{balanceOf(sender)}} & \tiny{0x2cda3fa1fffffffe000000020008007e87fe00001c180f800046f383eb594355}\\ 
\sourcecode{\_receivers.length} & 3 \\ 
\sourcecode{\_receivers[0]} & \sourcecode{ADDRS[2]} \\ 
\sourcecode{\_receivers[1]} & \sourcecode{ADDRS[2]} \\ 
\sourcecode{\_receivers[2]} & \sourcecode{ADDRS[0]} \\ 
\sourcecode{\_value} & \tiny{0xb380b590a3ff87ff3ffff9560000c3baaaad1d4a74e77a85be86c5459cf3a343}\\
\hline
\end{tabular}
\end{center}
\caption{Concrete example exploits the \sourcecode{batchTransfer()} function.}
\label{fig:concrete}
\end{figure}

Figure~\ref{fig:concrete} shows a concrete error triggering transaction
{\systemname} generates for exploiting the error we described in
Section~\ref{sec:example}.
% Appendix~\ref{appendix:error-triggering} presents a concrete example that
% {\systemname} generates to violate the total supply invariant. 
With the above
assignment, the security check \sourcecode{balances(msg.sender)>=amount} in
line 20 in Figure~\ref{code:BECToken} is bypassed and \sourcecode{msg.sender}
is able to send more tokens to receivers than it owns. After the execution of
\sourcecode{batchTransfer()}, the check condition at line 18 in
Figure~\ref{code:total} is violated. {\systemname} therefore successfully
detects and reports this error to the user.

==> files/appb.tex <==
\section{Memory Operations}\label{appendix:memory}
Figure~\ref{code:opt} shows an example of storing and loading memory data without
any optimization. To store a 256-bit integer \sourcecode{value}, a naive approach would 
first generate 32 \sourcecode{extract} instructions and 32 \sourcecode{store} instructions.
Each pair of \sourcecode{extract} and \sourcecode{store} instructions 
extract a 8-bit integer from \sourcecode{value} and 
store the integer to the memory.
Similarly, to load a 256-bit integer from memory, 
the system would generate 32 \sourcecode{select}
instructions to load a 256-bit integer from the memory. 
Each instruction loads a 8-bit integer from memory. 
It then would concatenate 32 8-bit integers into a 256-bit integer.

\begin{figure}[t]
\begin{center}
\inputminted
{Scheme}{code/load.smt2}
\end{center}
\caption{Constraints from MSTORE and MLOAD instructions without simplification.}
\label{code:opt}
\end{figure}


==> files/appc.tex <==
\section{Invariants and Constraints}\label{sec:constraints}

In this section, we describe how a user checks the 
invariants and the constraints using {\systemname}.

\begin{figure}[t]
\inputminted{Python}{./code/transfer.py}
\caption{Policies for transfer function.}
\label{code:transfer}
\end{figure}

\begin{figure}[t]
\inputminted{Python}{./code/approve.py}
\caption{Policies for approve and transferFrom functions (ERC-20).}
\label{code:approve}
\end{figure}

\begin{figure}[t]
\inputminted{Python}{./code/approve-nft.py}
\caption{Policies for approve and transferFrom functions (ERC-721).}
\label{code:approve-nft}
\end{figure}

\noindent{\textbf{Total Supply:}} As described in
Section~\ref{sec:example} and Figure~\ref{code:total},  ERC-20 tokens are
designed as assets that can be sent and received and in practice many 
ERC-20 tokens are traded publicly and have market value.  If the total supply changes
unexpectedly due to software errors, it may have significant impact on the
market value of each token.  We applied {\systemname} to check if any public
function in our benchmark contracts will break the total supply invariant.

\noindent\textbf{Transfer:} The \sourcecode{transfer()} function defines
the most fundamental functionality of an ERC-20 token, that allows a user to transfer his
balances to other users.  To secure a token transfer, the contract must
guarantee that the sender has enough token to transfer. Otherwise, the token
transfer should fail.

Figure \ref{code:transfer} shows the function to build transfer policy, 
where \sourcecode{acc[0]} and \sourcecode{acc[1]} are two symbolic accounts 
and \sourcecode{value} is a symbolic value. Before calling
the function \sourcecode{transfer()}, account \sourcecode{acc[0]} owns \sourcecode{pre\_bal[0]} tokens and \sourcecode{acc[1]} 
owns \sourcecode{pre\_bal[1]} tokens. \sourcecode{acc[0]} creates a transaction that transfers \sourcecode{value} 
tokens to \sourcecode{acc[1]}. \sourcecode{post\_bal[0]} and \sourcecode{post\_bal[1]} are tokens owned by \sourcecode{acc[0]}
and \sourcecode{acc[1]} after calling the \sourcecode{transfer()} function. At line 11-18, the generated
constraints check if the transfer function breaks the security rule defined above.

\noindent\textbf{Token Approval (ERC-20):} The \sourcecode{approve()} and
the \sourcecode{transferFrom()} functions allow a user to authorize a third party to
spend his token. A user calls the \sourcecode{approve()} function to allow a third
party to spend tokens in his account and the third party uses the
\sourcecode{transferFrom()} function to transfer the token.

Figure~\ref{code:approve} shows the security policies built for
\sourcecode{approve()} and \sourcecode{transferFrom()} scheme. At line 8 account
\sourcecode{acc[0]} calls the function \sourcecode{approve()} to authorize
\sourcecode{acc[2]} to spend up to \sourcecode{values[0]} tokens.
\sourcecode{acc[2]} then calls the \sourcecode{transferFrom} function to transfer
\sourcecode{acc[0]}'s token to \sourcecode{acc[1]}'s account.

A secure \sourcecode{transferFrom()} transaction should check the following
conditions. 1) \sourcecode{acc[0]} has enough tokens to perform the
transaction; 2) the transferred token is smaller than \sourcecode{acc[0]}'s
allowance; 3) the allowance and the account balances should be updated
correspondingly if the transfer succeeds (line 15-26).

\noindent\textbf{Token Approval (ERC-721):}
Similar to ERC-20, ERC-721 allows a user to transfer his ownership of a token
to other users.  Different from ERC-20, ERC-721 uses the \sourcecode{approve()} function to
authorize a third party to transfer a single token and
\sourcecode{setApprovalForAll} to authorize a third party to manage all
assets.

In Figure~\ref{code:approve-nft}, {\systemname} assumes that \sourcecode{acc[0]} is not
authorized to transfer token \sourcecode{tid} and \sourcecode{acc[1]} is not the owner
of \sourcecode{tid} (line 5-12). \sourcecode{acc[0]} then creates a transaction that transfers the ownership 
of \sourcecode{tid} from \sourcecode{owner} to \sourcecode{acc[1]} (line 13). A vulnerable contract would
allow the transaction and modify the ownership correspondingly.


==> files/appd.tex <==
\section{Experiment Results}\label{appendix:examples}

\noindent\textbf{Backdoor:} To allocate tokens on the fly, many tokens
implement a mint function that allows the contract admin to issues new tokens to
others.  However, missing security checks may leave backdoors that allow the
contract admin to modify balances of other accounts to an arbitrary number.
Figure \ref{code:ATL} shows the mint function from ATL \footnote{contract
address: 0x78b7fada55a64dd895d8c8c35779dd8b67fa8a05}. The \sourcecode{mint()} function allows
the contract owner to allocate tokens to an address \sourcecode{\_holder}. The
function first verifies that the transaction is from contract owner (line 2),
and the value is not zero (line 3). The contract sets a token limit that the
total supply of this token should not be more than \sourcecode{TOKEN\_LIMIT}
(line 4). The function then updates the balance of \sourcecode{\_holder} and
\sourcecode{totalSupply}.

\begin{figure}[t]
\inputminted{JavaScript}{./code/atl.sol}
\caption{The ATL contract code snippet.}
\label{code:ATL}
\end{figure}

{\systemname} found two issues from this function.  Suppose the owner calls
\sourcecode{mint()} with a large \sourcecode{\_value}.  First, the guard that
token's total supply should less than \sourcecode{TOKEN\_LIMIT} can be bypassed
by an overflow attack.  This allows the owner to allocate more tokens than the
contract allows. Second, \sourcecode{\_holder}'s balance can be overflowed and
can be set to any number at line 5. This effectively allows  the owner to
change a user's balance to an arbitrary number (e.g., to confiscate tokens from
a user).

\begin{figure}[t]
\inputminted{JavaScript}{./code/rex.sol}
\caption{The simplified RexToken code snippet.}
\label{code:rex}
\end{figure}

\noindent\textbf{Attackable:} 
Figure \ref{code:rex} shows the \sourcecode{migrate()} and
\sourcecode{claimMigrate()} function from RexToken\footnote{contract address:
    0xf05a9382A4C3F29E2784502754293D88b835109C}. Those two functions allow
RexToken users to migrate their tokens stored in previous contracts to this
contract. While executing the \sourcecode{claimMigrate() function}, it
increases the balance of the sender and the total supply of the token
respectively without any overflow check at lines 7 and 8. {\systemname} marks
this contract as vulnerable because the total supply invariant can be violated
if the sender has large amount of token in previous contract.  Although this is
theoretically exploitable, we investigated these two contracts on Etherscan
main chain and such exploitations are not possible with the current contract
state.

\begin{figure}[t]
\inputminted{JavaScript}{./code/paragon.sol}
\caption{The ParagonCoinToken code snippet.}
\label{code:paragon}
\end{figure}

\noindent\textbf{Deviation:} 
Figure \ref{code:paragon} shows the simplified \sourcecode{transfer()} function
from ParagonCoinToken\footnote{contract address:
0x7728dFEF5aBd468669EB7f9b48A7f70a501eD29D}. Unlike other ERC-20 tokens,
ParagonCoinToken computes a transaction fee each time a user transfer tokens to
the other (line 6-7), which breaks the transfer policy that all tokens should
be transferred to receiver's account. We believe this a deviation from ERC-20
standard. Note that a user can change the constraint to avoid treating this
constraint as vulnerable if desired.

\begin{figure}[t]
\inputminted{JavaScript}{./code/fp.sol}
\caption{The PRASMToken code snippet.}
\label{code:fp}
\end{figure}

\noindent\textbf{False Positive:} Figure~\ref{code:fp} shows the \sourcecode{balanceOf()} function from
PRASMToken\footnote{contract address:
    0x1a66e09f7dccc10eae46e27cfa6b8d44a50df1e7}. {\systemname} reports that
this contract may break the specified constraints if an integer overflow occurs
when computing the balance at line 8 in Figure~\ref{code:fp}. This is
unfortunately a false positive because the total supply of this contract is
fixed as a constant after being initialized during the contract construction at line
4. Therefore, the sum of \sourcecode{balances[\_holder]} and
\sourcecode{lockupBalance} at line 8 will never overflow. 


\noindent\textbf{Error Disclosure:} RexToken is only theoretically attackable but not exploitable given 
its current state. ATL and ParagonCoinToken correspond to an owner backdoor and a standard deviation 
case, respectively. For these three errors, disclosing these contracts clearly aligns with the 
stakeholder/public interest.

==> files/appe.tex <==
\section{EVM Bytecode}

\noindent\textbf{Indirect Jump:} One difference between EVM and the core
language in Section~\ref{sec:design} is that the jump instructions in EVM are
indirect, i.e., an EVM jump instruction fetches the jump target address from
the execution stack.  To handle such jump instructions, {\systemname} checks
whether the destination from the stack is symbolic. If so, {\systemname} gets
all possible values from the SMT solver and forks the current execution state
for each jump destination.  In practice, the current implementation of the Solidity
compiler guarantees that the jump destination is always constant.

\noindent\textbf{Miscellaneous Blockchain State:} Global blockchain states such
as timestamp and block height are initialized as fresh symbolic variables.  This
is consistent with the fact that a transaction may occur at any time and any
state in Ethereum.  {\systemname} updates these state values accordingly when
new transactions are generated. Each transaction is assigned with enough gas to
execute and {\systemname} leverages the gas limit system so that the system will stop
after certain iterations.

